Double excitation energies from quantum Monte Carlo using state-specific energy optimization

We show that recently developed quantum Monte Carlo methods, which provide accurate vertical transition energies for single excitations, also successfully treat double excitations. We study the double excitations in medium-sized molecules, some of which are challenging for high level coupled-cluster calculations to model accurately. Our fixed-node diffusion Monte Carlo excitation energies are in very good agreement with reliable benchmarks, when available, and provide accurate predictions for excitation energies of difficult systems where reference values are lacking.

==> appendices/supp_info.tex <==
\begin{suppinfo}
Choice of input weights for the matching of multiple CIPSI wave functions; CIPSI energies, PT2 energies, and variances for the expansions used in the QMC calculations; additional QMC total and excitation energies obtained with CAS wave functions and with CIPSI determinantal components originally expressed in a CAS orbital basis.
\end{suppinfo}


==> supplementary_information/cipsi-process-fig.tex <==
\begin{figure}[htb]
\begin{center}
\includegraphics[scale=0.342]{cipsi-process-fig}
\caption{\label{fig:cipsi-process} Breakdown of the CIPSI calculation process. The process always begins with the MCSCF orbitals (red lines) from a CASSCF calculation (in GAMESS) which are used as the MO basis in Quantum Package. Next, for nitroxyl, glyoxal, and tetrazine, a full-CI including doubles (FCID) with zero seniority is performed. For cyclopentadienone an iterative CISD is performed up to $N_{\mathrm{det}}^{\mathrm{max}}\sim10^3$. The expansion is then truncated to between 2$-$100 determinants, depending on the system. Finally, an unrestricted CIPSI is performed up to $N_{\mathrm{det}}^{\mathrm{max}}\sim10^2-10^4$. The expansion and MCSCF orbitals are used in CHAMP for the VMC optimization and DMC calculations. Alternatively, the natural orbitals (NO) are generated and the CIPSI process is repeated (dark yellow lines). The new expansion and orbitals are then used in CHAMP.}
\end{center}
\end{figure}


==> supplementary_information/glyoxal/glyoxal-overlap-fig.tex <==
\begin{figure}[htb]
\begin{center}
%\includegraphics[scale=0.3]{fig-overlap-fixed-lambda.pdf}
%\includegraphics[scale=0.3]{fig-overlap-varying-lambda.pdf}
\includegraphics[scale=0.4]{glyoxal-overlap-lambda.pdf}
	\caption{\label{fig:glyoxal-overlap} The effective overlap between the ground- and excited-state wave function ($|S_{12}|^2$) of glyoxal [CIPSI (NO) 5046 determinants (see Table~\ref{tab:glyoxal-SI})] plotted throughout the SR optimization for different values of $\lambda_{12}$. The sampling at a given step increases as $t_{\mathrm{SR}}$ increases.}
\end{center}
\end{figure}

% 1. Make font larger
% 2. Change 'lambda' in key to Greek symbol
% 3. The y axis label should be defined outside the plot as something simpler, then used in the image instead of the explicit form.
% 4. Add A), B), or something?
% 5. Add a line for the initial overlap for all. 3.724459205732803E-008
% 6. Change colors, don't use yellow

% should really do this on a different system, with a small expansion, quickly to see if the same thing occurs. It is weird the ground-state changes but not the excited state. Why would the GS ever increase in energy? Well, if the energy surface found sees the higher energy as the mimnima at that SR step.


==> supplementary_information/si-title.tex <==
\title{Supporting Information: Accurate double excitation energies using penalty-based quantum Monte Carlo optimization}


